Learning to update Auto-associative Memory in Recurrent Neural Networks for Improving Sequence Memorization

Learning to remember long sequences remains a challenging task for recurrent neural networks. Register memory and attention mechanisms were both proposed to resolve the issue with either high computational cost to retain memory differentiability, or by discounting the RNN representation learning towards encoding shorter local contexts than encouraging long sequence encoding. Associative memory, which studies the compression of multiple patterns in a fixed size memory, were rarely considered in recent years. Although some recent work tries to introduce associative memory in RNN and mimic the energy decay process in Hopfield nets, it inherits the shortcoming of rule-based memory updates, and the memory capacity is limited. This paper proposes a method to learn the memory update rule jointly with task objective to improve memory capacity for remembering long sequences. Also, we propose an architecture that uses multiple such associative memory for more complex input encoding. We observed some interesting facts when compared to other RNN architectures on some well-studied sequence learning tasks.

==> cover_letter.tex <==
%\documentclass[letterpaper]{article} %DO NOT CHANGE THIS
%\begin{document}
Dear reviewer:
\\

Thanks very much for your interest in this paper. This paper were submitted to NIPS 2017, and was not ready by then. I hope this could be a pleasant read this time after significant revision. 
\\

The paper was attacked mainly on writing. The experiments are sound, but writing was not polished. \\

The major problem of writing was that the intuition and the reason why the networks work is not well presented. The paper had many experiments, but it has to be cut to fit the page limit, so a lot of introduction were cut off, which seriously hurt the paper readability and idea flow. The intuition on the networks design was not well explained, so that reviewers were to fill in the blank, which is not always easy for all the readers. 
\\

In this version, we fixed all those problems. Specifically, the understanding and the thought process has been addressed with clarity in introduction, especially, the relationship to associative memory such as Hopfield nets, Boltzmann Machines, as well as recent fast weights work were clearly explained. 
\\

More details on experiments were put in and intuitions on how our RNN could handle them well is explained theoretically as well as empirically.
\\

Due to those changes, we have to cut off some experiments. However, we attached one of the abandoned experiment into appendix, which also shows much better results than the previous NIPS submission thanks to a bug fix.
\\

I am confident that the current version is in a much better shape, and it should have the material, as well as the presentation quality for AAAI. 
\\


%\end{document}
